Are Gross Substitutes a Substitute for Submodular Valuations?

The class of gross substitutes (GS) set functions plays a central role in Economics and Computer Science. GS belongs to the hierarchy of {\em complement free} valuations introduced by Lehmann, Lehmann and Nisan, along with other prominent classes: $GS \subsetneq Submodular \subsetneq XOS \subsetneq Subadditive$. The GS class has always been more enigmatic than its counterpart classes, both in its definition and in its relation to the other classes. For example, while it is well understood how closely the Submodular, XOS and Subadditive classes (point-wise) approximate one another, approximability of these classes by GS remained wide open. Our main result is the existence of a submodular valuation (one that is also budget additive) that cannot be approximated by GS within a ratio better than $\Omega(\frac{\log m}{\log\log m})$, where $m$ is the number of items. En route, we uncover a new symmetrization operation that preserves GS, which may be of independent interest. We show that our main result is tight with respect to budget additive valuations. Additionally, for a class of submodular functions that we refer to as {\em concave of Rado} valuations (this class greatly extends budget additive valuations), we show approximability by GS within an $O(\log^2m)$ factor.

==> app-sym-lb.tex <==
%\subsection{Factor $\sim 2$ Gap between GS and Budget-Additive}

In Section~\ref{sec:factor2-sep} we establish a factor 2 gap with respect to BA functions using the greedy characterization of GS functions. 
In this section we re-derive this gap using the symmetrization technique.
%(The result in Section~\ref{sec:log-ba} is stronger than the result presented here; we present it mainly to demonstrate the applicability of the symmetrization technique).

Recall that the BA function $f$ considered in Proposition~\ref{prop:approx-2} has one item $a$ of value~1, and $k$ items $b_1, \ldots, b_k$, each of value $1/k$. Its budget is~1.
Note that $f$ is precisely $BA(k,1)$ (per Definition~\ref{def:ba-k-d}).

\begin{theorem}
	$BA(k,1)$ cannot be approximated by GS within a ratio better than $\frac{2k}{k+1}$.
\end{theorem}

\begin{proof}
	Let $f=BA(k,1)$. 
	We show that no GS function that respects the symmetries of $f$ approximates $f$ within a ratio better than $\frac{2k}{k+1}$. 
	Let $g$ be a GS function that respects the symmetries of $f$.
	Let $B$ denote the set of items $b_1, \ldots, b_k$.
	For simplicity of presentation, we sometimes omit the parenthesis of sets when referring to singletons (i.e., denote $\{x\}$ by $x$).
	
	If $g(a)<\frac{k+1}{2k}$, then $\frac{f(a)}{g(a)}>\frac{2k}{k+1}$ and we are done.
	Hence we may assume that $g(a)\geq \frac{k+1}{2k}$. 
	Since all sets have value at most~1, $g(B \mid a) \leq \frac{k-1}{2k}$.
	Let $B_2 = B \setminus \{b_1\}$.
	Observe that $g(B_2 \mid a) \leq g(B \mid a) \leq \frac{k-1}{2k}$. 
	By Lemma~\ref{lem:key}, $g(B_2 \mid b_1) \le g(B_2 \mid a)$.
	In addition, $g(b_1) \le \frac{1}{k}$.
	We get $g(B) = g(b_1) + g(B_2 \mid b_1) \leq \frac{1}{k} + \frac{k-1}{2k} = \frac{k+1}{2k}$, whereas $f(B) = 1$.
\end{proof}

%%\subsection{Factor $\sqrt{m}$ Gap between GS and XOS}
%%
%%\begin{proposition}
%%	\label{pro:XOS}
%%	If $m$ is a perfect square, then XOS cannot be approximated by GS within a ratio better than $\sqrt{m}$.
%%\end{proposition}
%%
%%
%%\begin{proof}
%%	Items are partitioned into $\sqrt{m}$ groups $M_1, \dots, M_{\sqrt m}$, each of size $\sqrt{m}$. The XOS function is $f = \max_i\{f_i\}$, where $f_i$ is additive (with item values~1) over the $i$th group.
%%	We show that no GS function that respects the symmetries of $f$ approximates $f$ within a ratio better than $\sqrt m$. 
%%	
%%	Let $g$ be a GS function that respects the symmetries of $f$. Let $T$ be a set with one item from each group (all such sets $T$ have the same value by symmetry), and observe that $g(T) \le f(T) = 1$.
%%Consider a random item $x\in T$ and a random permutation $\pi$ over the items of $T$. The expected (expectation taken both over choice of $x$ and choice of $\pi$) marginal value of $x$ (marginal value compared to the prefix of $\pi$ that precedes $x$) is exactly $\frac{g(T)}{|T|} \le \frac{1}{\sqrt{m}}$. Consequently, there exists an item $x\in T$, for which the above expectation (now taken only over choice of $\pi$) is at most $\frac{1}{\sqrt{m}}$. Consider the group $M_i$ that $x$ belongs to. By Proposition~\ref{pro:GSisSWS}, the marginal contribution of the $j$th item to $g(M_i)$ is not larger than the marginal contribution of $x$ to $g(T)$ when $x$ is in the $j$th location. As there are $\sqrt{m}$ locations and the expected contribution at a random location (corresponding to the random permutation $\pi$) is at most $\frac{1}{\sqrt{m}}$, we have that $g(M_i) \le 1$. But $f(M_i) = \sqrt{m}$, showing that the approximation ratio cannot be better than $\sqrt{m}$.  
%%\end{proof}
%%
%%\noindent {\bf Remark:} It is known that submodular functions do not approximate $f$ of Proposition~\ref{pro:XOS} within a ratio better than $\Omega(\sqrt m)$, but they do achieve a ratio somewhat better than $\sqrt{m}$. For example, when $m=4$ the submodular function that is~$\frac{2}{3}$ on sets of size~1, is~$\frac{4}{3}$ on sets of size~3 or more, and either~1 or~$\frac{4}{3}$ on sets of size~2 (the latter holding if both items are from the same group), gives a $\frac{3}{2} < 2$ approximation. Hence Proposition~\ref{pro:XOS} does not follow from known results.



==> app-threshold-previous-proof.tex <==
In this section we prove Proposition~\ref{prop:h-GS}.

\begin{proof}
	We first show that $h$ is monotone, i.e., that $h(a \mid S)\geq 0$ for every set $S$ and item $a$. By adding $a$ last in the sorted order of $S$, a non-negative value is added to $h$. Then, keep swapping $a$ with its neighbor until it reaches its place (according to $g$). By Claim~\ref{cl:exchange}, each such swap cannot decrease $h$.
	
	We next show that $h$ is submodular. 
	It suffices to prove that for every set $S$ and two items $a,b$, $h(b \mid S) \geq h(b \mid Sa)$.
	Adding an item $j$ to a set $T$ has two effects: (i) the value goes up by the marginal value of $j$ w.r.t. its position within $T$, denote this position $r$, (ii) the value goes down by the sum, over all items positioned $r$ or higher, of the difference in the marginal values due to the shift in position.
	Let $r$ and $q$ be the respective positions of items $a$ and $b$ when added to $S$, and let $k=|S|$. 
	We distinguish between two cases, as follows.
	
	\noindent {\bf Case 1:} $g(a) \ge g(b)$. In this case $b$'s position when added to $Sa$ is $q+1$. The respective marginal values of $b$ with respect to $S$ and $Sa$ are
	\begin{eqnarray*}
	h(b \mid S) & = & \mu(b,q) - \sum_{i=q}^{k}\left(\mu(S_{i},i) - \mu(S_{i},i+1)\right)\\
	h(b \mid Sa) & = & \mu(b,q+1) - \sum_{i=q}^{k}\left(\mu(S_{i},i+1) - \mu(S_{i},i+2)\right).
	\end{eqnarray*}
	We need to show that $h(b \mid S) - h(b \mid Sa) \geq 0$.
	{\footnotesize
		\begin{eqnarray}
		h(b \mid S) - h(b \mid Sa) & = & \mu(b,q)-\mu(b,q+1)-\left(\mu(S_q,q) - \mu(S_q,q+1) \right) \nonumber\\
		& + & \sum_{i=q}^{k-1} \left(\mu(S_{i},i+1)-\mu(S_{i},i+2)-\left(\mu(S_{i+1},i+1)-\mu(S_{i+1},i+2)\right)\right) \nonumber\\
		& + & \mu(S_k,k+1)-\mu(S_k,k+2).
		\label{eq:sm-case1}
		\end{eqnarray}
	}
	The first two lines of (\ref{eq:sm-case1}) are non-negative by Claim~\ref{cl:exchange}, and the last line is non-negative by the monotonicity of $T$.
	
	\noindent {\bf Case 2:} $g(a) < g(b)$. In this case $b$'s position when added to $Sa$ is still $q$. The respective marginal values of $b$ with respect to $S$ and $Sa$ are
	\begin{eqnarray*}
	h(b \mid S) & = & \mu(b,q) - \sum_{i=q}^{k}\left(\mu(S_{i},i) - \mu(S_{i},i+1)\right)\\
	h(b \mid Sa) & = & \mu(b,q) - \sum_{i=q}^{r-1}\left(\mu(S_{i},i) - \mu(S_{i},i+1)\right) - \left(\mu(a,r) - \mu(a,r+1)\right) - 
	\sum_{i=r}^{k}\left(\mu(S_{i},i+1) - \mu(S_{i},i+2)\right).
	\end{eqnarray*}
	We need to show that $h(b \mid S) - h(b \mid Sa) \geq 0$.
	{\footnotesize
		\begin{eqnarray}
		h(b \mid S) - h(b \mid Sa) & = & \mu(a,r)-\mu(a,r+1)-\left(\mu(S_r,r) - \mu(S_r,r+1) \right) \nonumber\\
		& + & \sum_{i=r}^{k-1} \left(\mu(S_{i},i+1)-\mu(S_{i},i+2)-\left(\mu(S_{i+1},i+1)-\mu(S_{i+1},i+2)\right)\right) \nonumber\\
		& + & \mu(S_k,k+1)-\mu(S_k,k+2).
		\label{eq:sm-case2}
		\end{eqnarray}
	}
	The first two lines of (\ref{eq:sm-case2}) are non-negative by Claim~\ref{cl:exchange}, and the last line is non-negative by the monotonicity of $T$.
	
	It remains to show that $h$ satisfies the triplet condition; that is, for every set $S$, and 3 items $a,b,c$, 
	$$
	h(a \mid S)+h(bc \mid S) \leq \max\{h(b \mid S)+h(ac \mid S),h(c \mid S)+h(ab \mid S)\}.
	$$
	Assume without loss of generality that $g(a)\geq g(b) \geq g(c)$. 
	We show that 
	\begin{equation*}
	\label{eq:triple}
	h(a \mid S)+h(bc \mid S) = h(b \mid S)+h(ac \mid S) \geq h(c \mid S)+h(ab \mid S).
	\end{equation*}
	
	Let $q$ (resp., $t$) be the position of item $b$ (resp., $c$) when added to $S$, and let $k = |S|$.
	
	We first show that $h(a \mid S)+h(bc \mid S) = h(b \mid S)+h(ac \mid S)$, or equivalently, that $h(c \mid Sb) = h(c \mid Sa)$.
	Indeed, $h(c \mid Sb) = h(c \mid Sa) = \mu(c,t) + \sum_{i=t}^{k} \left(\mu(S_{i},i+1) - \mu(S_{i},i+2)\right)$.
	
	We next show that $h(a \mid S)+h(bc \mid S) \geq h(c \mid S)+h(ab \mid S)$, or equivalently, that $h(b \mid S) - h(b \mid Sa) + h(c \mid Sb) - h(c \mid S) \geq 0$. 
	After canceling out terms, we get
	\begin{eqnarray}
	& & h(b \mid S) - h(b \mid Sa) + h(c \mid Sb) - h(c \mid S)  = \nonumber \\ 
	& & \mu(b,q)-\mu(b,q+1)-\left(\mu(S_q,q) - \mu(S_q,q+1)\right) + \nonumber\\
	& & \sum_{i=q}^{t-2} \left( \mu(S_{i},i+1)-\mu(S_{i},i+2) - \left(\mu(S_{i+1},i+1) - \mu(S_{i+1},i+2)\right) \right) + \nonumber\\
	& & \mu(S_{t-1},t)-\mu(S_{t-1},t+1) - \left(\mu(c,t)-\mu(c,t+1)\right) \geq 0 \nonumber,
	\label{eq:trip}
	\end{eqnarray}
	where the last inequality follows since every line in this expression is non-negative by Claim~\ref{cl:exchange}; this concludes the proof of Proposition~\ref{prop:h-GS}.
\end{proof}

==> app-threshold.tex <==
In this section we prove Proposition~\ref{prop:h-GS}.

\begin{proof}
Consider a bipartite graph $G(M,V;E)$ with $|V| = |M|$ and with non-negative weights on the edges, whether for every $j \in M$ and $r \in V$, the weight of edge $(j,r)$ is $\mu(j,r)$ (with $\mu$ as in the definition of $h$). Let $h'$ be the set function where for every $S \subset M$, $h'(S)$ is the total weight of the maximum weight matching on the subgraph induced by $S$ and $V$. Then by definition (see Definition~\ref{def:oxs}) $h'$ is an OXS function. We show below that for every set $S\subset M$, $h(S) = h'(S)$, concluding that $h$ is an OXS function, and hence monotone and GS, proving Proposition~\ref{prop:h-GS}.

Consider an arbitrary $S \subset M$, and recall that $h(S) = \sum_{r=1}^{|S|} \mu(S_r,r)$. Consider the matching $MS$ that for every $1 \le r \le |S|$ matches item $S_r\in M$ with vertex $r \in V$. Claim~\ref{cl:exchange} implies that $MS$ is a maximum weight matching on the subgraph induced by $S$ and $V$. Consequently $h'(S) = \sum_{r=1}^{|S|} \mu(S_r,r) = h(S)$, as desired.
\end{proof}




==> symmetry-app.tex <==
In this section we prove Lemma~\ref{lem:twoItemSymmetrization}. 

Let $h$ be the two-item max-symmetrization function introduced in Definition~\ref{def:max-symmetrization}.
We show that if $h$ is applied to a monotone GS function, the resulting function is a monotone GS function. % dominated by $f$.
%The proof is separated into multiple lemmas. 
%Monotonicity and domination by $f$ are proved in Lemma \ref{lem:monotone}.
Monotonicity is proved in Lemma \ref{lem:monotone}, submodularity is proved in Lemma \ref{lem:h-sm}, and the triplet condition is proved in Lemma \ref{lem:h-triplet}.

\begin{lemma}
	\label{lem:monotone}
	The function $h$ is monotone.% and is dominated by $f$.
\end{lemma}

\begin{proof}
	%We first show that $h$ is monotone. 
	Consider sets $S,T \subseteq M$ such that $S \subseteq T$. We need to show that $h(T) \ge h(S)$.
	If $\{a,b\} \in S$ or $\{a,b\} \cap S = \phi$, then $h(S) = g(S)$, and the monotonicity of $h$ follows because $h(T) \ge g(T) \ge g(S)$.
	It remains to handle the cases in which $|\{a,b\} \cap S| = 1$.
	
	Suppose that $S=S'a$ and $T=T'a$ such that $S' \subseteq T'$, and $b\not\in T'$.
	It holds that
	$$
	h(S) = \max\{g(S'a),g(S'b)\}\leq \max\{g(T'a),g(T'b)\}=h(T),
	$$
	where the inequality follows by the monotonicity of $g$.
	
	For the case where $S=S'a$ and $T=T'ab$ with $S' \subseteq T'$, we get
	$$
	h(S) = \max\{g(S'a),g(S'b)\}\leq \max\{g(T'a),g(T'b)\} \leq g(T'ab) = h(T).
	$$
	
	
%	We next show that $h$ is dominated by $f$.
%	Let $S \subseteq M$. If $|S \cap \{a,b\}|\neq 1$, then $h(S)=g(S)\leq f(S)$.
%	If $|S \cap \{a,b\}|= 1$, suppose w.l.o.g. that $S=S'a$. We get
%	$$
%	h(S)=\max\{g(S'a),g(S'b)\}\le \max\{f(S'a),f(S'b)\} = f(S'a),
%	$$
%	where the inequality follows by $f$ dominating $g$, and the last equality follows from $f$ being $(a,b)$-symmetric.
%	%	If $g(a \mid S') \geq g(b \mid S')$, then $h(S) = g(S'a) \leq f(S'a) = f(S)$.
%	%	Else, by symmetry of $f$ we get $h(S) = g(S'b) \leq f(S'b) = f(S'a) = f(S)$.
\end{proof}

\begin{lemma}
	\label{lem:h-sm}
	The function $h$ is submodular.
\end{lemma}

\begin{proof}%[Proof of Lemma~\ref{lem:h-sm}]
	
	To prove submodularity, it suffices to prove that for every set $S$ and every two items $c,d \not\in S$, it holds that $h(c|S) \ge h(c|Sd)$. The following four cases can be addressed without using the fact that $g$ is GS.
	
	\begin{enumerate}
		
		\item If $\{a,b\} \subset S$ then the claim follows from the submodularity of $g$, and the fact that $h=g$ for the sets of interest.
		
		\item If $\{a,b\} \cap S = \phi$ there are several subcases to consider:
		
		\begin{enumerate}
			
			\item If $d \not\in \{a,b\}$ and $c \not\in \{a,b\}$, the claim follows from the submodularity of $g$, and the fact that $h=g$ for the sets of interest.
			
			\item If $d \not\in \{a,b\}$ and $c \in \{a,b\}$ (w.l.o.g., $c = a$), the claim follows because $h(a|S) = \max\{g(a|S),g(b|S)\} \geq \max\{g(a|Sd),g(b|Sd)\} = h(a|Sd)$, where the inequality follows by submodularity of $g$.
			
			\item If $d \in \{a,b\}$ and $c \not\in \{a,b\}$, suppose without loss of generality that $g(Sac) \ge g(Sbc)$. Then the claim follows because $h(c|S) = g(c|S) \geq g(Sac) - g(Sa) \ge g(Sac) - \max\{g(Sa),g(Sb)\} = h(c|Sa)$, where the last equality follows from $g(Sac) \ge g(Sbc)$.
			
			\item If $d \in \{a,b\}$ and $c \in \{a,b\}$, suppose without loss of generality that $g(Sa) \ge g(Sb)$. Then the claim follows because for $c \in \{a,b\}$ we have that $h(c|S) = \max\{g(a|S),g(b|S)\} \ge g(b|S) \geq g(b|Sa) \ge g(Sab) - \max\{g(Sa),g(Sb)\} = h(c|Sd)$, where the last equality follows from $h(Sd) = \max\{g(Sa),g(Sb)\}$.
			
		\end{enumerate}
		
		\item If $|\{a,b\} \cap S| = 1$ (w.l.o.g., $a \subset S$, and we let $S = S'a$) and $d=b$, then $h(c|Sb) = g(c|Sb)$ (as $S = S'a$). If $g(S'a) \ge g(S'b)$ the claim follows because then $h(c|S) \ge g(c|S) \ge g(c|Sb) = h(c|Sb)$.
		If $g(S'b) \ge g(S'a)$, the claim follows because then $h(c|S) \ge g(S'bc) - g(S'b) = g(c|S'b) \ge g(c|Sb) = h(c|Sb)$.
		
		
		
		\item If $|\{a,b\} \cap S| = 1$ (w.l.o.g., $a \subset S$) and $c=b$, let $S = S'a$. Then $h(b|S) = \min\{g(b|S'a), g(a|S'b)\}$ whereas $h(b|Sd) = \min\{g(b|S'ad), g(a|S'bd)\}$. The claim follows by submodularity of $g$.
		
	\end{enumerate}
	
	It remains to deal with the case that $|\{a,b\} \cap S| = 1$ (w.l.o.g., $a \subset S$, and we let $S = S'a$) and $b \not \in \{c,d\}$. This is the only case in which we will need to use the fact that $g$ is not only submodular, but also GS. The following claim addresses this case. For simplicity of notation (but without affecting the proof), its formulation assumes that $S' = \phi$.
	
	%One can verify that it is sufficient to prove the two following claims.
	
	%\begin{claim}
	%	The function $h$ satisfies $h(a|S) \geq h(a|T)$ for every $S,T$ such that $S \subseteq T$ and $b \not\in T$.
	%\end{claim}
	
	%\begin{proof}
	%	It holds that $h(a|S) = \max\{g(a|S),g(b|S)\} \geq \max\{g(a|T),g(b|T)\} = h(a|T)$, where the inequality follows by submodularity of $g$.
	%\end{proof}
	
	
	
	\begin{claim}
		\label{claim:last-case-sm}
		The function $h$ satisfies $h(c \mid a) \geq h(c \mid da)$.
	\end{claim}
	
	\begin{proof}
		Based on the definition of $h$, proving the claim amounts to proving that
		\begin{equation}
		\label{eq:submod}
		\underbrace{\max\{g(ac),g(bc)\}+\max\{g(ad),g(bd)\}}_{\text{LHS}} \geq \underbrace{\max\{g(acd),g(bcd)\}+\max\{g(a),g(b)\}}_{\text{RHS}}.
		\end{equation}
		
		For each term of the form $\max\{g(aS),g(bS)\}$ we say that $a$ realizes the max term if $g(aS) \geq g(bS)$; otherwise, we say that $b$ realizes the max term.
		%
		We distinguish between the following cases. Case 1 is addressed without using the fact that $g$ is GS. The remaining cases use this fact.
		
		The first cases are ones where either (i) $a$ realizes both max terms in the RHS of \eqref{eq:submod}, or (ii) $b$ realizes both max terms in the RHS of \eqref{eq:submod}. We establish \eqref{eq:submod} for (i) (case 1 below); (ii) is proved analogously.
		
		{\bf Case 1:} $g(acd) \geq g(bcd)$ and $g(a) \geq g(b)$. We get:
		$$
		g(acd)+g(a) \leq g(ac) + g(ad) \leq \max\{g(ac),g(bc)\}+\max\{g(ad),g(bd)\},
		$$
		where the first inequality follows by submodularity.
		
		The next cases are ones where $a$ realizes exactly one of the max terms in the LHS of \eqref{eq:submod}, and exactly one of the max-terms in the RHS of \eqref{eq:submod}. We establish \eqref{eq:submod} for the cases where $a$ realizes the first max term of LHS (cases 2,3 below); the other two cases are proved analogously.
		
		{\bf Case 2:}
		(i) $g(ac)\geq g(bc)$, (ii) $g(bd) > g(ad)$, (iii) $g(a)\geq g(b)$ and (iv) $g(bcd)\geq g(acd)$.
		Suppose toward contradiction that Equation \eqref{eq:submod} is violated. That is, (v) $g(ac) + g(bd) < g(a) + g(bcd)$. Then, by submodularity we get
		\begin{equation}
		\label{eq:11}
		g(ac)-g(a) < g(cd) - g(d).
		\end{equation}
		We get: $g(bc)+g(ad) < g(ac)+g(bd) < g(a)+g(bcd)$, where the first inequality follows from (i) and (ii), and the second inequality is (v).
		By submodularity it follows that $g(ad)+g(c) < g(a)+g(cd)$. By the triplet condition w.r.t. $acd$, it follows that $g(d)+g(ac) = g(a)+g(cd)$, in contradiction to Equation \eqref{eq:11}.
		
		%		{\bf Case 3:} (i) $g(ac)\geq g(bc)$, (ii) $g(bd) > g(ad)$, (iii) $g(b)\geq g(a)$ and (iv) $g(acd)\geq g(bcd)$.
		%		This case is similar to Case 2 and is deferred to Appendix~\ref{sec:app-symmetric}.
		
		{\bf Case 3:} (i) $g(ac)\geq g(bc)$, (ii) $g(bd) > g(ad)$, (iii) $g(b)\geq g(a)$ and (iv) $g(acd)\geq g(bcd)$.
		Suppose toward contradiction that Equation \eqref{eq:submod} is violated. That is, (v) $g(ac) + g(bd) < g(b) + g(acd)$. Then, by submodularity we get
		\begin{equation}
		\label{eq:111}
		g(bd)-g(b) < g(cd) - g(c).
		\end{equation}
		We get: $g(bc)+g(ad) < g(ac)+g(bd) < g(b)+g(acd)$, where the first inequality follows from (i) and (ii), and the second inequality is (v).
		By submodularity it follows that $g(bc)+g(d) < g(b)+g(cd)$. By the triplet condition w.r.t. $bcd$, it follows that $g(c)+g(bd) = g(b)+g(cd)$, in contradiction to Equation \eqref{eq:111}.
		
		
		The remaining cases are ones where either (i) $a$ realizes both max terms in the LHS of \eqref{eq:submod}, and exactly one of the max terms in the RHS, or (ii) $b$ realizes both max terms in the LHS of \eqref{eq:submod}, and exactly one of the max terms in the RHS. We establish \eqref{eq:submod} for the two cases of (i) (cases 4,5 below); the two cases of (ii) are proved analogously.
		
		{\bf Case 4:} (i) $g(ac)\geq g(bc)$, (ii) $g(ad) \geq g(bd)$, (iii) $g(a)\geq g(b)$ and (iv) $g(bcd) > g(acd)$.
		Suppose toward contradiction that Equation \eqref{eq:submod} is violated. That is, (v) $g(ac) + g(ad) < g(a) + g(bcd)$. Then, by (i), (v) and submodularity we get
		\begin{equation*}
		g(ad)-g(a) < g(cd) - g(c)
		\end{equation*}
		Consequently, by the triplet condition w.r.t. $acd$ we get
		\begin{equation}
		\label{eq:1111}
		g(ad)+g(c) < g(ac) + g(d).
		\end{equation}
		
		Similarly, by (ii), (v) and submodularity we get
		\begin{equation*}
		g(ac)-g(a) < g(cd) - g(d)
		\end{equation*}
		Consequently, by the triplet condition w.r.t. $acd$ we get $g(ac)+g(d) < g(ad) + g(c)$, contradicting \eqref{eq:1111}.
		
		%		{\bf Case 5:} (i) $g(ac)\geq g(bc)$, (ii) $g(ad) \geq g(bd)$, (iii) $g(a) < g(b)$ and (iv) $g(acd) \geq g(bcd)$.
		%		This case is similar to Case 4 and is deferred to Appendix~\ref{sec:app-symmetric}.
		
		{\bf Case 5:} (i) $g(ac)\geq g(bc)$, (ii) $g(ad) \geq g(bd)$, (iii) $g(a) < g(b)$ and (iv) $g(acd) \geq g(bcd)$.
		
		Suppose toward contradiction that Equation \eqref{eq:submod} is violated. That is, (v) $g(ac) + g(ad) < g(b) + g(acd)$. Then, by (i), (v) and submodularity we get
		\begin{equation*}
		g(bc)-g(b) < g(cd) - g(d).
		\end{equation*}
		Consequently, by the triplet condition w.r.t. $bcd$, we get
		\begin{equation}
		g(bc)+g(d) < g(bd) + g(c)
		\label{eq:11111}
		\end{equation}
		
		Similarly, by (ii), (v) and submodularity we get
		\begin{equation*}
		g(bd)-g(b) < g(cd) - g(c).
		\end{equation*}
		Consequently, by the triplet condition w.r.t. $bcd$, we get $g(bd)+g(c) < g(bc) + g(d)$, contradicting \eqref{eq:11111}
	\end{proof}	
	This concludes the proof of Lemma~\ref{lem:h-sm}.
\end{proof}


\begin{remark}
	\label{rem:notSubmodular}
	There exists a monotone submodular function $g$ on $4$ items such that the induced $h$ function is not submodular. That is, the triplet condition of $g$ is necessary for submodularity of $h$. To see this, consider the following function:
	$g(\emptyset)=0,
	g(a)=3,
	g(b)=2,
	g(c)=1,
	g(d)=2,
	g(ab)=5,
	g(ac)=3,
	g(ad)=3,
	g(bc)=3,
	g(bd)=4,
	g(cd)=3,
	g(abc)=5,
	g(abd)=5,
	g(acd)=3,
	g(bcd)=5,
	g(abcd)=5
	$.
	One can verify that $g$ is submodular, but $h(c|a)=0$ while $h(c|da)=1$, violating submodularity.
\end{remark}

\begin{lemma}
	\label{lem:h-triplet}
	The function $h$ satisfies the triplet condition of GS.
\end{lemma}

\begin{proof}
	The triplet condition involves a base set $S$, and a triple $T$ of three items that are not in $S$. 
	There are five cases to consider (see below). Among the five, four are quite simple to address. In contrast, the fifth case is not easy to establish, and we prove it by a computer assisted code.
	
	\begin{itemize}[noitemsep]
		\item $\{a,b\} \cap (S \cup T) = \phi$. In this case the triplet condition for $h$ follows from that for $g$.
		\item $|\{a,b\} \cap S| = 2$. In this case the triplet condition for $h$ follows from that for $g$.
		\item $|\{a,b\} \cap T| = 2$. This case is handled in Claim~\ref{claim:T2}.% in Appendix~\ref{sec:app-symmetric}.
		\item $|\{a,b\} \cap T| = 1$ and $|\{a,b\} \cap S| \in \{0,1\}$. This case is handled in Claim~\ref{claim:T1S01}.% in Appendix~\ref{sec:app-symmetric}.
		\item $|\{a,b\} \cap T| = 0$ and $|\{a,b\} \cap S| = 1$. This case is handled in Claim~\ref{claim:S1}, via a computer assisted proof.	
	\end{itemize}
	\vspace{-0.3in}
\end{proof}

\begin{claim}
	\label{claim:T2}
	Let $S$ be a set s.t. $S \cap \{a,b\} = \emptyset$. Then, $h$ satisfies the triplet condition for every triple $T$ with $\{a,b\}\subset T$.
\end{claim}

\begin{proof}
	Observe that $h(a \mid S) = h(b \mid S) = \max\{g(a \mid S), g(b \mid S)\}$ and that $h(bc \mid S) = h(ac \mid S) = \max\{g(ac \mid S), g(bc \mid S)\}$. Consequently  $h(a \mid S)+h(bc \mid S) = h(b \mid S)+h(ac \mid S)$. Hence it suffices to prove that 	$h(c \mid S)+h(ab \mid S) \le \max\{h(a \mid S)+h(bc \mid S),h(b \mid S)+h(ac \mid S)\}$. The last inequality is verified as follows:
	\begin{eqnarray*}
		h(c \mid S)+h(ab \mid S) & = & g(c \mid S)+g(ab \mid S)\\
		& \leq & \max\{g(a \mid S)+g(bc \mid S),g(b \mid S)+g(ac \mid S)\}\\
		& \leq & \max\{h(a \mid S)+h(bc \mid S),h(b \mid S)+h(ac \mid S)\},
		%& = & g(c \mid S) + \max\{g(a \mid S)+g(b \mid Sc),g(b \mid S)+g(a \mid Sc)\}\\
		%& \leq & g(c \mid S) + \max\{g(a \mid S),g(b \mid S)\} + \max\{g(a \mid Sc),g(b \mid Sc)\},
	\end{eqnarray*}
	where the first inequality follows by the triplet condition w.r.t. $abc$.
\end{proof}

\begin{claim}
	\label{claim:T1S01}
	Let $S,T$ be sets such that $|\{a,b\} \cap T|=1$ and $|\{a,b\} \cap S| \in \{0,1\}$. Then, $h$ satisfies the triplet condition.
\end{claim}

\begin{proof}
	Given a set $S$ and triple $T = \{x,y,z\}$, there are the following three {\em pairs}:
	$(Sx, Syz)$, $(Sy, Sxz)$, $(Sz, Sxy)$. Suppose that in each of the three pairs, exactly one of the two terms contains exactly one item from $\{a,b\}$. This is indeed the case when $|\{a,b\} \cap T| = 1$, where if $|\{a,b\} \cap S| = 0$ the other term in the pair is disjoint from  $\{a,b\}$, whereas if $|\{a,b\} \cap S| = 1$ the other term in the pair contains both $a$ and $b$. Consider a table with three rows and three columns. Each column corresponds to one of the pairs. For $j \in \{1,2,3\}$, the $j$th entry in the first row gives the sum of values of $g$ applied to the two terms in the $j$th pair, when the item from $\{a,b\}$ (in the term that has one such item) is taken to be $a$. The entries in the second row are constructed in an analogous way, with $a$ replaced by $b$. The third row corresponds to values under $h$, hence each of its entries is the maximum among the two other entries in its column. Let $M$ denote the maximum value in this table. $M$ must appear in at least one of the first two rows, and by the triplet property of $g$, it must appear at least twice in that row. Consequently, it appears at least twice also in the third row, implying the $h$ satisfies the triplet condition.	
\end{proof}



\begin{claim}
	\label{claim:S1}
	Let $S,T$ be such that $|\{a,b\} \cap T| = 0$ and $|\{a,b\} \cap S| = 1$. Then, $h$ satisfies the triplet condition.
\end{claim}

\begin{proof}
	We first observe that it is sufficient to prove the claim for the case of 5 items. Indeed, if there is a counterexample consisting of a triplet $T$ and a base set $S$, then the function $h'$ defined as $h'(X)=h(X \mid S\setminus \{a,b\})$ (i.e., the marginal value with respect to $S \setminus \{a,b\}$), defined over $T \cup \{a,b\}$, would also serve as a counterexample. (It is known that GS is closed under marginal value; i.e., if $h$ is GS, then $h'$ is GS as well; this follows easily by Lemma~\ref{lem:triplet-char}.)
	
	Thus, without loss of generality we need to prove that
	$$
	h(c \mid a)+h(de \mid a) \leq \max\{h(d \mid a)+h(ce \mid a), h(e \mid a)+h(cd \mid a)\},
	$$
	or equivalently,
	$$
	h(ca)+h(dea) \leq \max\{h(da)+h(cea), h(ea)+h(cda)\}.
	$$
	We say that a term of the form $h(aS)$ is realized by $a$ if $g(aS) \geq g(bS)$; otherwise, we say that it is realizes by $b$.
	%
	Observe that if either $a$ realizes both terms in the left hand side or $b$ realizes both terms, then the inequality follows by the triplet condition for $g$.
	Thus, it remains to show that the inequality holds when one of these terms is realizes by $a$ and the other is realized by $b$. Without loss of generality assume that $h(ca)=g(ca)$ and $h(dea)=g(deb)$. We need to show that
	\begin{equation}
	g(ca)+g(deb) \leq \max\{h(da)+h(cea), h(ea)+h(cda)\}.
	\label{eq:desired}
	\end{equation}
	Recall that each one of the 4 terms of the form $h(Sa)$ in the RHS of~\eqref{eq:desired} is realized by either $a$ or $b$.
	
	A counterexample to Inequality~\eqref{eq:desired} takes the form of an {\em instantiation of $g$}, where an instantiation of $g$ is a function that assigns a value $g(B)$ to every non-empty subset $B \subseteq \{a,b,c,d,e\}$ in such a way that $g$ is GS (i.e., satisfies monotonicity, submodularity and the triplet condition), and $g$ has the property that applying two-item max-symmetrization to the items $a$ and $b$ results in a function $h$ that violates Inequality~\eqref{eq:desired}.
	A violation of Inequality~\eqref{eq:desired} is encoded by 8 strict linear inequalities, namely
	$g(ca)+g(deb) > g(d\ast)+g(ce\ast)$, and $g(ca)+g(deb) > g(e\ast)+g(cd\ast)$, for $\ast \in \{a,b\}$. We refer to these inequalities as the 8 fixed constraints.
	
	To show that no counterexample exists, it is sufficient to show that there does not exist an instantiation of $g$ that satisfies the triplet condition, and also the 8 fixed constraints. 
	
	We actually prove a stronger result, but let us first introduce some additional notation.
	A {\em combination} is a tuple of a triplet from $\{a,b,c,d,e\}$ and a base set from the remaining two items. 
	Let $(ijk;S)$ denote the combination consisting of the triplet $\{i,j,k\}$ and the base set $S$ (if $S$ is a singleton $\{\ell\}$ we write $(ijk;\ell)$ for simplicity).
	For $g$ to satisfy the triplet condition, it should satisfy the triplet inequality (\ref{eq:no-unique-max}) for a total of 40 combinations ($\binom{5}{3}=10$ possible triplets, and 4 possible base sets for every triplet). 
	We show that even the more modest requirement to satisfy the triplet condition with respect to only 6 (particular) combinations leads to a contradiction.
	In particular, we show the following:
	
	\begin{claim}
		\label{cl:infeasible}
		There does not exist an instantiation of $g$ that satisfies the 8 fixed constraints, and the triplet condition with respect to the following 6 combinations: $(acd;b),(ace;b),(ade;b),(bce;a),(bde;a),(cde;b)$.\footnote{The same claim holds with respect to the following 6 combinations as well: $(acd;e),(ace;d),(ade;c),(bcd;e),(bce;d),(cde;a)$.}
	\end{claim}
	
	We prove this claim by a linear programming-based computer assisted code. The code is now available in GitHub~\cite{github}.
	Claim~\ref{cl:infeasible} implies Inequality~\eqref{eq:desired}, which concludes the proof of Claim~\ref{claim:S1}.
	Readers who are interested in more details about the LP-based code are referred to Subsection~\ref{sec:code}.
	\end{proof} 
	
\subsection{The LP-Based Code}
	\label{sec:code}
	In this section we give details regarding the code used to prove Claim~\ref{cl:infeasible}. 
	
%	Recall that $g$ should satisfy the triplet inequality for each combination.
	We wish to encode the fact that $g$ satisfies the triplet condition using linear inequalities. 
	For each combination, there are 3 ways to choose the minimum  out of the 3 terms (recall, the maximum should not be unique). Every such choice can be encoded by one equality and one weak inequality.
	
	For example, consider the combination $(abd;e)$. For this combination, the minimum term is either (i) $g(a \mid e) + g(bd \mid e)$, (ii) $g(b \mid e) + g(ad \mid e)$, or (iii) $g(d \mid e) + g(ab \mid e)$. To encode that, say, $g(d \mid e) + g(ab \mid e)$ is a minimum, we write:
	$$
	g(a \mid e) + g(bd \mid e) \geq g(d \mid e) + g(ab \mid e) \quad \mbox{ and } \quad g(b \mid e) + g(ad \mid e) = g(a \mid e) + g(bd \mid e).
	$$
	
	A naive implementation would run $3^{40}$ linear programs, each with 31 variables (one for each non-empty subset of $\{a,b,c,d,e\}$) and 88 linear constraints (the 8 fixed constraints\footnote{Recall that these constraints are strict inequalities. In the LP, we encoded a strict inequality of the form $x > y$ by the weak inequality $x \geq y+1$. One can verify that this choice does not affect the feasibility of the LP.} for the violation of Inequality~\eqref{eq:desired}, plus 80 constraints, 2 for each one of the 40 combinations).
	
	To overcome the associated computational challenge, our code gradually grows a ternary tree of height 40, where each node corresponds to a combination, the three edges from a given node correspond to the 3 ways to choose the minimum term of that combination, and each combination appears in all nodes in a given level of the tree.
	%Let $h_v$ denote the height of node $v$.
	%We gradually build the set of LPs as follows.
	A node $v$ of height $h$ is associated with an LP with $8+2h$ constraints, corresponding to the 8 fixed constraints and the $2h$ constraints corresponding to the path from $v$ to the root. A feasible solution to the LP of a leaf node corresponds to an instantiation of $g$ that satisfies the triplet condition and violates  Inequality~\eqref{eq:desired}.
	
	Thus, a necessary condition for violating the assertion of Claim~\ref{claim:S1} is a leaf node whose corresponding LP is feasible. Consequently, to prove the claim it suffices to prove that no such leaf exists. We grow the tree from the root (using BSF/DSF), and once infeasibility is obtained for a node $v$, we trim off its subtree and backtrack.
	The advantage of growing the tree gradually is that some branches of the tree may be trimmed off early on, substantially reducing the number of LPs that we need to solve.
	Note that the order of the 40 combinations may be crucial in determining the runtime of the program. Indeed, we observe high variability in the  depth reached by different orders.
	
	We ran two different implementations of the program, written by two different programmers, one in matlab, the other in C++.
	The full code is available in GitHub~\cite{github}.
	The program terminated without finding any feasible leaf, concluding the proof of Claim~\ref{claim:S1}. The best order resulted in a search of depth 6 (i.e., 6 combinations). Interestingly, there are exactly two (out of $\binom{40}{6} > 3.8$ million) sets of 6 combinations that suffice to trim off the entire tree (thereby conclude that no feasible leaf exists), and no set of 5 combinations suffices. The two sets of 6 combinations are the ones specified in Claim~\ref{cl:infeasible}, namely: (1) $\{(acd;b),(ace;b),(ade;b),(bce;a),(bde;a),(cde;b)\}$, (2) $\{(acd;e),(ace;d),(ade;c),(bcd;e),(bce;d),(cde;a)\}$.



